Autonomous Block Assembly for Boom Cranes with Passive Joint Dynamics: Integrated Vision MPC Control

This paper presents an autonomous control framework for articulated boom cranes performing prefabricated block assembly in construction environments. The key challenge addressed is precise placement control under passive joint dynamics that cause pendulum-like sway, complicating the accurate positioning of building components. Our integrated approach combines real-time vision-based pose estimation of building blocks, collision-aware B-spline path planning, and nonlinear model predictive control (NMPC) to achieve autonomous pickup, placement, and obstacle-avoidance assembly operations. The framework is validated on a laboratory-scale testbed that emulates crane kinematics and passive dynamics while enabling rapid experimentation. The collision-aware planner generates feasible B-spline references in real-time on CPU hardware with anytime performance, while the NMPC controller actively suppresses passive joint sway and tracks the planned trajectory under continuous vision feedback. Experimental results demonstrate autonomous block stacking and obstacle-avoidance assembly, with sway damping reducing settling times by more than an order of magnitude compared to uncontrolled passive dynamics, confirming the real-time feasibility of the integrated approach for construction automation.

==> full_code.tex <==

\begin{abstract}
This paper presents a unified perception–planning–control framework for under-actuated manipulators with passive joints, motivated by articulated boom cranes in construction. 
The framework integrates vision-based pose estimation, collision-free path generation, and nonlinear model predictive control (nonlinear MPC) into a closed loop that achieves real-time execution of assembly tasks. 
A laboratory-scale testbed emulates crane kinematics and passive dynamics, enabling rapid experimentation while providing a path toward transfer to full-scale machinery. 
The planner generates collision-free B-spline references with anytime performance on a CPU, while the NMPC stabilizes passive joint sway and advances along the path under online vision updates. 
Experiments demonstrate autonomous block pickup, placement, and obstacle-avoidance assembly, confirming real-time feasibility and showing that sway damping reduces settling times by more than an order of magnitude. 
The results highlight laboratory-scale testbeds as effective enablers for developing autonomy concepts for large-scale construction equipment.
\end{abstract}



\section{Introduction}
The construction industry remains one of the least digitized sectors, facing labor shortages, safety risks, and limited automation \cite{XiC22a, GhC20, MeW20, ZhC25a}. Unlike manufacturing, construction must operate in unstructured, variable environments that complicate the deployment of robotic systems. Robotic assembly of prefabricated components (RAC) has emerged as a promising direction, yet existing systems are typically restricted to single tasks and lack adaptability to complex on-site conditions \cite{GhC20, ChA25}.  

A central challenge arises from the use of \emph{large-scale, under-actuated manipulators} such as articulated boom cranes. Passive joints reduce structural load but introduce swing dynamics that degrade positioning accuracy, making precise assembly difficult. Robust autonomy therefore requires (i) online vision-based pose estimation of building elements, (ii) active sway damping under passive dynamics, and (iii) collision-free path planning in cluttered, contact-rich environments. Existing approaches typically address these aspects in isolation, limiting applicability to real construction sites \cite{ZhC25a}.  

To address this gap, we develop and evaluate a \emph{laboratory-scale framework} that integrates perception, planning, and nonlinear MPC (NMPC) control in a unified closed loop. The platform emulates the kinematics and under-actuated dynamics of articulated boom cranes while enabling rapid experimentation under controlled conditions. The long-term vision is to transfer this framework to full-scale construction machinery. Figure~\ref{fig:titlepage} illustrates both the motivating crane scenario and the developed lab setup. A video of the experiments is available at \url{LINK_REMOVED_FOR_ANONYMITY}.


\begin{figure}[t]
    \centering
    \includegraphics[width=80mm, height=45mm]{graphics/motivation.png}
    \caption{Motivation: articulated boom crane with suspended block (left) and developed laboratory-scale setup (right) as a testbed for autonomous assembly.}
    \label{fig:titlepage}
\end{figure}

\subsection{Related Work}
Research on under-actuated manipulators spans several domains relevant to articulated boom cranes.  

\textbf{Control of under-actuated systems.} Early approaches converted passive-joint constraints into equivalent input constraints for linear MPC formulations \cite{ZhS23}, while more recent nonlinear MPC (NMPC) schemes directly incorporate passive dynamics \cite{KaB14, ScA23b}. Flatness-based MPC achieved sway suppression with low computational cost \cite{ScA23b}, but lacked flexibility for constraint handling and path-following. Reinforcement learning has shown operator-level performance in large-scale material handling \cite{SpE24a}, yet training requirements and generalization issues limit deployment to unstructured construction sites \cite{HeJ24}.  

\textbf{Forestry and construction cranes.} Forestry cranes, structurally similar to articulated boom cranes, have been widely used as experimental platforms. Dynamic programming methods achieved up to \SI{90}{\percent} sway reduction in simulation and experimental testbeds \cite{JeS23, JeS25, Jebellat2025}. NMPC implementations demonstrated accurate tracking with oscillation reductions of \SI{59}{\percent} to \SI{76}{\percent} \cite{KaB14}. In construction contexts, advanced modeling using screw theory has been applied for force analysis in articulated jib cranes \cite{AmG22, CiE19}, while trajectory optimization with hydraulic constraints achieved near time-optimal, collision-free motions in simulation \cite{EcB25}.  

\textbf{Integration with perception.} Vision-based feedback has been applied in knuckle-boom crane control using multi-camera systems for simultaneous payload damping and parameter estimation \cite{TyC21}. However, these works treat vision and control as separate problems, typically assuming pre-computed reference trajectories. Robotic assembly in construction (RAC) has achieved successes with perception-integrated pipelines for loading tasks \cite{AyF24a}, yet remains focused on industrial manipulators in structured scenarios, not large-scale under-actuated systems.  

\textbf{Research gap.} Despite these advances, no existing framework combines vision-based pose estimation, collision-free path planning, and NMPC-based sway damping in a closed loop for articulated boom cranes. Bridging this gap requires laboratory-scale testbeds that emulate large-scale under-actuated dynamics while enabling rapid experimentation. This motivates the framework developed in this work.

\subsection{Contributions}
The main contribution of this work is a unified framework and laboratory testbed for developing autonomous control of large-scale, under-actuated manipulators such as articulated boom cranes. Specifically:
\begin{itemize}
    \item \textbf{Integrated perception–planning–control architecture:} Real-time vision feedback, collision-free path generation, and nonlinear MPC are combined in a single closed loop that accounts for passive joint dynamics and provides active sway damping.  
    \item \textbf{Laboratory-scale validation:} A physical testbed emulating articulated crane dynamics is used to demonstrate autonomous pick-and-place and obstacle-avoidance assembly. The experiments confirm the framework’s real-time feasibility and its ability to suppress passive-joint sway by more than an order of magnitude, establishing a foundation for transfer to full-scale machinery.  
\end{itemize}


\subsection{Paper's Structure}
\cref{sec:modelling} introduces the dynamic model of articulated boom cranes with passive joints.  
\cref{sec:control} formulates the nonlinear MPC for path following and sway damping.  
\cref{sec:path_planning} presents the stochastic sampling-based planner for collision-free B-spline paths, followed in \cref{sec:pose_estimation} by the RGB/Aruco-based vision pipeline with filtering for online pose updates.  
\cref{sec:laboratory_setup} details the lab-scale setup, including low-level robot control and integration with the MPC.  
\cref{sec:results} reports experimental block assembly and quantifies the sway damping achieved by the controller.  
Finally, \cref{sec:conclusion} summarizes contributions and discusses scaling to full-size machinery.


\section{Modelling}
\label{sec:modelling}
The 9-DoF system is depicted on the right side of \cref{fig:system_overview}. 
It consists of the lightweight industrial robot \kuka with seven actuated DoFs, a cardan joint (passive joint) comprised of two non-actuated DoFs, and the Robotiq 2F-85 gripper. 
The design of the non-actuated joints resembles a forestry crane \cite{AnG19} equipped with a passive joint, which is commonly used to reduce stress on the mechanical construction induced by the load. 

\begin{figure*}[t]
    \centering
    % \input{graphics/system_block_diagram} 
    % \includegraphics[width=180mm,height=50mm]{example-image-a}
    \def\svgwidth{\textwidth} % relative width
    \import{graphics/overview}{overview_tex.pdf_tex}
    \caption{System overview. Left: schematic of the laboratory setup with robot, passive wrist joint, gripper, blocks, and reference frames $\mathcal{0}$ (base), $\mathcal{E}$ (end-effector), $\mathcal{T}$ (tool center), and $\mathcal{C}$ (camera). Right: block diagram of the integrated framework, illustrating the interconnection of perception, path planning, MPC control, and the environment model. The task sequencer executes pickup and placement routines based on a TOML configuration file specifying the schedule.}
    \label{fig:system_overview}
\end{figure*}

The equations of motion of the 9-DoF system with the generalized coordinates $\transpose{\vec{q}} = {[q_1, \dots, q_9]}$ can be written as
\begin{equation}
    \vec{M}(\vec{q}) \Ddot{\vec{q}} + \vec{C}(\vec{q},\dot{\vec{q}}) \dot{\vec{q}} + \vec{g}(\vec{q}) = \vec{\tau}
    \label{eq:eq_of_motion}
\end{equation}
with the mass matrix $\vec{M}(\vec{q})$, the Coriolis matrix $\vec{C}(\vec{q},\dot{\vec{q}})$, the gravitational forces $\vec{g}(\vec{q})$, and the generalized forces $\vec{\tau}$ \cite{SiS09, LyP17}.
For further consideration, the nine DoFs are split up into actuated $\transpose{\vec{q}_\text{a}} = {[q_1, \dots, q_7]}$ and non-actuated $\transpose{\vec{q}_\text{u}} = {[q_8, q_9]}$ DoFs. 
Based on this separation, \cref{eq:eq_of_motion} can be rearranged as
\begin{equation}
    \begin{bmatrix}
        \vec{M}_\text{a} & \vec{M}_\text{au} \\
        \vec{M}_\text{ua}& \vec{M}_\text{u} 
    \end{bmatrix}
    \begin{bmatrix}
        \Ddot{\vec{q}}_\text{a} \\
        \Ddot{\vec{q}}_\text{u}
    \end{bmatrix}
    +
    \begin{bmatrix}
        \vec{C}_\text{a} & \vec{C}_\text{au} \\
        \vec{C}_\text{ua} & \vec{C}_\text{u}
    \end{bmatrix}
    \begin{bmatrix}
        \dot{\vec{q}}_\text{a} \\
        \dot{\vec{q}}_\text{u}
    \end{bmatrix}
    +
    \begin{bmatrix}
        {\vec{g}}_\text{a} \\
        {\vec{g}}_\text{u}
    \end{bmatrix}
    =
    \begin{bmatrix}
        {\vec{\tau}}_\text{a} \\
        {\vec{0}}
    \end{bmatrix}
    \FullStop
    \label{eq:split_system}
\end{equation}
Considering the bottom line of \cref{eq:split_system}, the dynamics of the non-actuated system can be represented as
\begin{equation}
    \Ddot{\vec{q}}_\text{u} = {\vec{M}}_\text{u}^{-1} \left( -{\vec{M}}_\text{ua} \Ddot{\vec{q}}_\text{a} - {\vec{C}}_\text{ua} \dot{\vec{q}}_\text{a} - {\vec{C}}_\text{u} \dot{\vec{q}}_\text{u} - {\vec{g}}_\text{u} \right) \FullStop
    \label{eq:full_ua_dyn}
\end{equation}
In order to reduce the complexity of the model \cref{eq:full_ua_dyn}, the Coriolis terms $\vec{C}_\text{ua} \dot{\vec{q}}_\text{a}$ and $\vec{C}_\text{u} \dot{\vec{q}}_\text{u}$ are neglected as their contribution to the system dynamics is minor; see \cite{VuH21b}. This yields the simplified dynamics of the non-actuated system
\begin{equation}
    \Ddot{\vec{q}}_\text{u} = {\vec{M}}_\text{u}^{-1} \left( -{\vec{M}}_\text{ua} \Ddot{\vec{q}}_\text{a} - {\vec{g}}_\text{u} \right) \FullStop
    \label{eq:ua_dyn}
\end{equation}

It is further assumed that the actuated joints are controlled by a sub-ordinate controller such that the system input $\vec{u}$ for the receding horizon trajectory planning can be chosen as $\vec{u} = \ddot{\vec{q}}_\text{a}$. The resulting system dynamics are
\begin{equation}
\dot{\vec{x}} = \vec{f}(\vec{x},\vec{u}) = 
    \begin{bmatrix}
        \dot{\vec{q}}_\text{a} \\
        \dot{\vec{q}}_\text{u} \\
        \vec{u} \\
        {\vec{M}}_\text{u}^{-1} \left( -{\vec{M}}_\text{ua} {\vec{u}} - {\vec{g}}_\text{u} \right)
    \end{bmatrix} \Comma
\label{eq:sysdyn}
\end{equation}
with the system state $\transpose{\vec{x}} = [\transpose{\vec{q}}, \transpose{\dot{\vec{q}}}]$.

\subsection{Inverse Kinematics and Steady State of the Under-actuated System}
Due to the under-actuated dynamics, inverse kinematics solutions for goal points must correspond to steady states of the non-actuated subsystem to avoid unwanted swing motions. At steady state, both accelerations $\ddot{\vec{q}}_\text{u}$ and velocities $\dot{\vec{q}}_\text{u}$ of the under-actuated joints are zero.

From \cref{eq:ua_dyn}, the steady-state condition requires
\begin{equation}
    \vec{g}_\text{u}(\vec{q}) = \vec{0} \Comma
\end{equation}
where $\vec{g}_\text{u}(\vec{q})$ represents the gravitational forces acting on the under-actuated joints.

The steady-state configuration $\vec{q}_\text{s}$ is obtained by solving:
\begin{align}
\label{eq:ik}
    \vec{q}_\text{s} = \arg \min_{\vec{q}} \; & \Big[ \norm{ \vec{p}(\vec{q}) - \vec{p}_\text{d} }_2^2 
    + w_{\text{rot}} \norm{ \transpose{\vec{R}}_\text{d} \vec{R}(\vec{q}) - \mathbf{I} }_\text{F}^2 \Big] \\
    & \text{s.t.} \quad \vec{g}_\text{u}(\vec{q}) = \vec{0} \nonumber
\end{align}
where $\norm{\cdot}_\text{F}$ denotes the Frobenius norm, $\mathbf{I}$ is the identity matrix, and $w_{\text{rot}} = 0.1$ is chosen empirically. The orientation error formulation follows \cite{Hu09}.
The optimization problem \cref{eq:ik} is solved with Ipopt \cite{WaB06a}.


\section{Path-Following MPC Incorporating Passive Joint Dynamics}
\label{sec:control}

The path-following MPC approach is formulated as a finite-horizon optimal control problem that simultaneously optimizes the path parameter progression and the system's motion along a predefined spline-based path. Due to the under-actuated nature of the system, only the gripper's position and yaw angle can be directly controlled, necessitating a 4D task space representation $\vec{\xi} = \transvec{x, y, z, \psi}$ where roll and pitch orientations are determined by the passive joint dynamics. 
To enable precise assembly operations, the MPC formulation incorporates the passive joint dynamics while advancing the Cartesian path. 

\subsection{Spline-Based Path Parameterization}
Task space path parameterization is preferred for assembly operations as it provides smoother end-effector trajectories than joint space paths, which introduce irregular Cartesian motions due to kinematic nonlinearities. The path parameter $s \in [0,1]$ represents progression along the 4D path defined by a B-spline 
\begin{equation}
    \vec{\xi}_{\text{ref}}(s) = \sum_{i=0}^{n_\text{cp}-1} \vec{c}_{i} B_{i,k}(s) \Comma
    \label{eq:pathspline}
\end{equation}
where $B_{i,k}(s)$ are B-spline basis functions of degree $k$, and each control point $\vec{c}_{i} = \transvec{x_i, y_i, z_i, \psi_i}$, $i=0, \dots, n_\text{cp}-1$ contains position and yaw information. 


\subsection{Optimal Control Problem Formulation}
The aim of our control strategy is twofold: Firstly, it should incorporate the under-actuated system dynamics while stabilizing the gripper, and secondly, it should progress the path. 
For this we augment the original system state $\vec{x}$ with the path parameter $s$ and its velocity $\dot{s}$ resulting the augmented system state
$ \bar{\vec{x}} = \transvec{ \transpose{\vec{q}}, \transpose{\dot{\vec{q}}}, s, \dot{s}} \in \mathbb{R}^{2n_q + 2}$, 
as well as the augmented system input comprising the acceleration of the seven actuated joints and the path parameter acceleration as input
$ \bar{\vec{u}} = \transvec{ \transpose{\vec{u}}, v} = \transvec{ \transpose{\ddot{\Vec{q}}_{\text{a}}}, \ddot{s}} \in \mathbb{R}^{n_{\text{a}} + 1}$

Based on \cref{eq:sysdyn} the augmented system dynamics result in
\begin{equation}
    \dot{\bar{\vec{x}}} = \bar{\vec{f}}(\bar{\vec{x}}, \bar{\vec{u}}) = \begin{bmatrix}
        \dot{\Vec{q}} \\
        \Vec{u} \\
        {\Vec{M}}_{\text{u}}^{-1} \left( -{\Vec{M}}_{\text{ua}} \Vec{u} - {\vec{g}}_{\text{u}} \right) \\
        \dot{s} \\
        v
    \end{bmatrix} \FullStop
    \label{eq:aug_dynamics}
\end{equation}

The optimal control problem for the path-following MPC is defined as
\begin{subequations}
    \begin{alignat}{2}
        &\min_{\substack{\bar{\vec{x}}_{1|n}, \dots, \bar{\vec{x}}_{N|n} \\ 
            \bar{\vec{u}}_{1|n}, \dots, \bar{\vec{u}}_{N-1|n}}} 
            &&\sum_{k=0}^{N-1} l \left(\bar{\vec{x}}_{k|n}, \bar{\vec{u}}_{k|n} \right) + m \left(\bar{\vec{x}}_{N|n} \right) \label{eq:ocp} \\
        & \quad \text{s.t.} \ &&\bar{\vec{x}}_{k+1|n} = \vec{F}(\bar{\vec{x}}_{k|n}, \bar{\vec{u}}_{k|n})  \label{eq:sys_constr}\\
        & \quad && \bar{\vec{x}}_{0|n} = \bar{\vec{x}}(t_n) \label{eq:ocp_init} \\
        & \quad && \bar{\vec{x}}^\text{-} \leq \bar{\vec{x}}_{k|n} \leq \bar{\vec{x}}^\text{+} ,\quad \bar{\vec{u}}^\text{-} \leq \bar{\vec{u}}_{k|n} \leq \bar{\vec{u}}^\text{+} 
        \label{eq:ocp_limit}
    \end{alignat}
\end{subequations}
where $n$ indicates the iteration of the OCP and $k=0 \ldots N$ refers to the shooting node over the prediction horizon with length $N$. The discrete-time system dynamics $\Vec{F}(\cdot)$ are obtained through implicit Runge-Kutta integration of \cref{eq:sysdyn}.
The state limits $\bar{\vec{x}}^\pm = \transvec{{\vec{q}}^{\pm}_\text{a}, {\vec{q}}^{\pm}_\text{u}, {\dot{\vec{q}}}^{\pm}_\text{a}, {\dot{\vec{q}}}^{\pm}_\text{u}, s^{\pm}, \dot{s}^{\pm}}$ and input limits $\bar{\vec{u}}^\pm = \transvec{\vec{u}^\pm, v^\pm} $ in \cref{eq:ocp_limit} ensure the physical feasibility of the motion by including the joint limits and velocity limits for the robot
${\vec{q}}^\pm_\text{a} = \pm \transvec{162, 114, 162, 114, 162, 114, 166}$ in \si{\degree}, 
${\vec{q}}^\pm_\text{u} = \pm \transvec{43, 43}$ in \si{\degree},
${\dot{\vec{q}}}^\pm_\text{a} = \pm \transvec{85, 85, 100, 75, 130, 135, 135}$ in \si{\degree\per\second},
${\dot{\vec{q}}}^\pm_\text{u} = \pm \transvec{50, 50}$ in \si{\degree\per\second},
$s^\text{+} = 1$, $s^\text{-} = 0$, $\dot{s}^\pm = \pm 1$ and $\vec{u}^\pm = \pm \vec{1}$, $v^\pm = \pm 1$.

The cost function in \cref{eq:ocp} is divided into the Lagrange cost $l \left(\bar{\vec{x}}_{k|n}, \bar{\vec{u}}_{k|n} \right)$ and the Mayer cost term $ m \left(\bar{\vec{x}}_{N|n} \right)$. 
The Lagrange cost consists of task space tracking, joint space regularization, and control effort minimization
% \begin{align}
%     l(\bar{\vec{x}}_{k|n}, \bar{\vec{u}}_{k|n}) &= \|\tilde{\vec{p}}(\vec{q}_{k|n})\|^2_{\vec{Q}_{\text{pos}}} + \|\tilde{\psi}(\vec{q}_{k|n})\|^2_{Q_{\text{rot}}} \nonumber \\
%     &\quad + \|\tilde{\vec{q}}_{k|n}\|^2_{\vec{Q}_{\vec{q}}} + \|\tilde{\dot{\vec{q}}}_{k|n}\|^2_{\vec{Q}_{\dot{\vec{q}}}} \nonumber \\
%     &\quad + \|\tilde{s}_{k|n}\|^2_{Q_s} + \|\tilde{\dot{s}}_{k|n}\|^2_{Q_{\dot{s}}} \nonumber \\
%     &\quad + \|\vec{u}_{k|n}\|^2_{\vec{R}_{\vec{u}}} + \|v_{k|n}\|^2_{R_v}
%     \label{eq:lagrange_cost}
% \end{align}
\begin{align}
    l(\bar{\vec{x}}_{k|n}, \bar{\vec{u}}_{k|n}) &= \|\tilde{\vec{p}}(\vec{q}_{k|n})\|^2_{\vec{Q}_{\text{pos}}} + \|\tilde{\psi}(\vec{q}_{k|n})\|^2_{Q_{\text{rot}}} \nonumber \\
    &\quad + \|\tilde{\vec{q}}_{k|n}\|^2_{\vec{Q}_{q}} + \|\tilde{\dot{\vec{q}}}_{k|n}\|^2_{\vec{Q}_{\dot{q}}} \nonumber \\
    &\quad + \|\tilde{s}_{k|n}\|^2_{Q_s} + \|\tilde{\dot{s}}_{k|n}\|^2_{Q_{\dot{s}}} \nonumber \\
    &\quad + \|\vec{u}_{k|n}\|^2_{\vec{R}_{u}} + \|v_{k|n}\|^2_{R_v}
    \label{eq:lagrange_cost}
\end{align}
with weighted norms $\norm{\cdot}_Q$. 

The task space errors $ \tilde{\vec{p}}(\vec{q}_{k|n}) = \vec{p}(\vec{q}_{k|n}) - \vec{p}_{\text{ref}}(s_{k|n})$ and $\tilde{\psi}(\vec{q}_{k|n}) = \psi(\vec{q}_{k|n}) - \psi_{\text{ref}}(s_{k|n})$ with the Cartesian position $\vec{p}(\vec{q}_{k|n})$ and the gripper's yaw angle $\psi(\vec{q}_{k|n})$ depend on the joint configuration through forward kinematics, while $\vec{p}_{\text{ref}}(s_{k|n})$, and $\psi_{\text{ref}}(s_{k|n})$ are obtained from the evaluation of the reference path parameterized as B-spline.
% The joint space and path parameter errors are defined similarily as $\tilde{\vec{q}}_{k|n} = \vec{q}_{k|n} - \vec{q}_{\text{ref}}(s_{k|n})$, $\tilde{\dot{\vec{q}}}_{k|n} = \dot{\vec{q}}_{k|n} - \dot{\vec{q}}_{\text{ref}}(s_{k|n})$
% and $\tilde{s}_{k|n} = s_{k|n} - s_{\text{ref}}$, $\tilde{\dot{s}}_{k|n} = \dot{s}_{k|n} - \dot{s}_{\text{ref}}$,
The joint-space regularization terms are defined relative to a nominal posture 
$\vec{q}_\text{nom}$ and zero velocity as 
$\tilde{\vec{q}}_{k|n} = \vec{q}_{k|n} - \vec{q}_\text{nom}$, 
$\tilde{\dot{\vec{q}}}_{k|n} = \dot{\vec{q}}_{k|n}$. 
The path-parameter tracking errors are 
$\tilde{s}_{k|n} = s_{k|n} - s_\text{ref}$ and 
$\tilde{\dot{s}}_{k|n} = \dot{s}_{k|n} - \dot{s}_\text{ref}$.

The Mayer cost term at the final stage $m \left(\bar{\vec{x}}_{N|n} \right)$ is similar to the Lagrange cost \cref{eq:lagrange_cost}, except without dependencies on the input $\bar{\vec{u}}$
% \begin{align}
%     m(\bar{\vec{x}}_{N|n}) &= \|\tilde{\vec{p}}(\vec{q}_{N|n})\|^2_{\vec{Q}_{e,\text{pos}}} + \|\tilde{\psi}(\vec{q}_{N|n})\|^2_{Q_{e,\text{rot}}} \nonumber \\
%     &\quad + \|\tilde{\vec{q}}_{N|n}\|^2_{\vec{Q}_{e,\vec{q}}} + \|\tilde{\dot{\vec{q}}}_{N|n}\|^2_{\vec{Q}_{e,\dot{\vec{q}}}} \nonumber \\
%     &\quad + \|\tilde{s}_{N|n}\|^2_{Q_{e,s}} + \|\tilde{\dot{s}}_{N|n}\|^2_{Q_{e,\dot{s}}} \FullStop
%     \label{eq:mayer_cost}
% \end{align}
The values of the weight matrices and MPC parameters are listed in \cref{sec:results}.

% Kinematic redundancy is resolved by penalizing deviations of non-crane-like joints with high weights in $\vec{Q}_{\vec{q}}$.

Kinematic redundancy is resolved by regularizing joints toward a nominal posture $\vec q_\text{nom}$ with large weights on non–crane-like DoFs in $\mathbf{Q}_q$, while $\mathbf{Q}_{\dot q}$ damps joint velocities. 
%We do not use a path-dependent joint reference $\vec q_\text{ref}(s)$; tracking is performed purely in task space $(x,y,z,\psi)$.


% The kinematic redundancy of the 9-DOF manipulator for the 4-DOF task requires management of nullspace motions. 
% Specific joints not present in typical articulated crane kinematics are assigned reference values $\vec{q}_{\text{ref}}$ with correspondingly high weights, effectively removing redundancy by constraining these degrees of freedom. 

\subsection{Real-Time Implementation}
The computational efficiency required for real-time control is achieved through several key implementation choices. Traditional Euler-Lagrange formulations to obtain the equations of motion result in large symbolic expressions that lead to prohibitively long compile times and most important high computational cost, often producing hundreds of megabytes of generated code, particularly for computing the computationally expensive Hessian matrix.
To address these challenges, the implementation utilizes the Recursive Newton-Euler Algorithm (RNEA) \cite{Fe08} as implemented in the Pinocchio library \cite{CaS19a}. This approach, combined with CasADi's automatic differentiation capabilities \cite{AnG19}, enables efficient computation of the robot dynamics and their derivatives. The seamless integration of CasADi with the ACADOS optimal control framework \cite{VeF22b} allows for automatic generation, compilation, and execution of optimized solver binaries.
The B-spline path parameterization is implemented using a custom CasADi-compatible library, ensuring efficient evaluation of reference trajectories and their derivatives within the optimization framework. 

The ACADOS-generated solver employs the Real-Time Iteration (RTI) algorithm optimized for real-time performance, using a single QP iteration per MPC cycle with HPIPM as the QP solver featuring partial condensing and maximum 20 internal iterations \cite{FrD20a}. The configuration includes warm starting for accelerated convergence, merit function backtracking for robust convergence, exact Hessian computation and implicit Runge-Kutta (IRK) integration for numerical stability. The computation times of \cref{eq:ocp} with the given framework are illustrated in \cref{fig:acados_stats}.

\section{Collision-Free Path Planning}
\label{sec:path_planning}
Path-following MPC requires collision-free task-space references that can be updated at control rates. 
For this purpose, we adopt a lightweight stochastic ensemble method for B-spline paths in the $4$-D task space $(x,y,z,\psi)$. 
The method is inspired by \cite{NgN21,TiM18} and builds on prior GPU-based work \cite{VuE25}. 
Here, we adapt the approach to a CPU-optimized implementation that achieves anytime performance within tens of milliseconds, 
making it suitable for closed-loop integration with MPC in the laboratory crane setup.


\subsection{Problem Formulation}
Let $\vec{\xi}(s;\vec{c})\in \mathbb{R}^4$ denote a B-spline curve of degree $k$ with clamped uniform knots and control points $\vec{c}=\big[\vec{c}0,\dots,\vec{c}{n_{\mathrm{cp}}-1}\big]$. Start and goal are fixed, $\vec{\xi}(0)=\vec{\xi}_s$, $\vec{\xi}(1)=\vec{\xi}_e$, while interior points adapt to avoid collisions and shorten the path. Unless otherwise stated, we use quadratic B-splines ($k=2$) in experiments, which balance smoothness and computational efficiency.

Candidates are parameterized by $K=n_{\mathrm{cp}}-2$ interior via points $\{\vec{v}_i\}_{i=1}^{K}$, with fixed endpoints $\vec{v}_0=\vec{\xi}_s$, $\vec{v}_{K+1}=\vec{\xi}_e$. 
Control points $\vec{c}$ are solved such that $\vec{\xi}(s_i)\!\approx\!\vec{v}_i$ at uniformly spaced parameters. 
Thus, \emph{via points} act as sampling anchors, while \emph{control points} are the actual optimization variables. 
In all experiments, we use $K=3$ via points (start, goal, and one interior), which represents the minimal configuration sufficient for collision avoidance in the considered assembly tasks while keeping the optimization lightweight. 
Exploring larger numbers of via points for more complex assembly scenarios is left for future work.

\subsection{Ensemble Sampling and Update}
The initial candidate is a straight line between start and goal:
\begin{equation}
  \vec{v}_i^{(0)}=\vec{\xi}_s+\tfrac{i}{K+1}\,(\vec{\xi}_e-\vec{\xi}_s),\quad i=0,\dots,K{+}1.
  \label{eq:init_linear}
\end{equation}
An ensemble $\mathcal{P}=\{\vec{\xi}^{(m)}\}_{m=0}^{M}$ is generated by perturbing the interior via points with Gaussian noise:
\begin{equation}
  \vec{v}_i^{(m)} \sim \mathcal{N}\!\big(\mu_i,\sigma_i^2 \I_4\big), \qquad i=1,\dots,K,
\end{equation}
where $\mu_i$ and $\sigma_i$ are the current mean and standard deviation for each via point.  
After evaluating all candidates, the best fraction $\rho$ (elites) is used to update $(\mu_i,\sigma_i)$ by exponential moving average:
\begin{equation}
\begin{aligned}
  \mu_i &\leftarrow (1-\eta)\mu_i + \eta \!\sum_{m\in\mathcal{E}} w_m \vec{v}_i^{(m)}, \\
  \sigma_i &\leftarrow \max\{\sigma_{\min},\ \gamma\sigma_i\} \Comma
\end{aligned}
\end{equation}
with normalized weights $w_m$, learning rate $\eta$, contraction factor $\gamma<1$, and floor $\sigma_{\min}$. This contracts the ensemble toward promising regions while maintaining exploration.

\subsection{Collision Evaluation and Selection}
Each candidate is discretized at $N_c$ samples, $s_j=\tfrac{j}{N_c-1}$, $j=0,\dots,N_c{-}1$. Feasibility is checked via MuJoCo’s collision pipeline \cite{todorov2012mujoco}. Among all collision-free candidates $\mathcal{P}^\star$, the one with minimum arc length
\begin{equation}
  L(\vec{\xi})=\sum_{j=1}^{N_c-1}\norm{\vec{\xi}(s_j)-\vec{\xi}(s_{j-1})}
\end{equation}
is selected as reference $\vec{\xi}_{\mathrm{ref}}^\star$.  
This path seeds the next iteration, enabling anytime refinement in closed-loop.

\subsection{Benchmark Results}
The planner was benchmarked on the crane scenario ($4$-DoF, $K=3$ via points). 
Table~\ref{tab:ces_bench} reports statistics over $N{=}50$ runs. 
All converged runs succeeded within $\approx 12$\,ms on average, while anytime runs 
show the expected trade-off: shorter budgets yield feasible but slightly longer 
paths, whereas increasing the budget steadily improves path quality. 
Notably, success rates remain near 100\% even under tight budgets, confirming 
robustness for real-time MPC.

\begin{table}[h]
\centering
\caption{Planner benchmark results over $N{=}50$ runs. 
``Converged'' refers to full optimization (60 iterations). 
``Anytime'' settings limit computation to the given budget, after which the best candidate is returned. 
Reported runtime is the actual wall-clock time (mean$\pm$std), while path length measures solution quality (lower is better).}
\label{tab:ces_bench}
\begin{tabular}{lccc}
\toprule
Setting & Success [\%] & Time [ms] & Avg. length [m] \\
\midrule
Converged (60 iters) & 100 & $12.3\pm6.3$ & 0.89 \\
Anytime 10 ms & 94--98 & $15.5\pm3.7$ & 0.80 \\
Anytime 20 ms & 98 & $25.2\pm3.2$ & 0.67 \\
Anytime 50 ms & 100 & $54.5\pm3.0$ & 0.59 \\
\bottomrule
\end{tabular}
\end{table}


\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{graphics/ensemble_init.png}
        \caption{Initial ensemble of candidate B-splines, sampled around the straight-line initialization.}
        \label{fig:ensemble_init}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{graphics/ensemble_iter10.png}
        \caption{Ensemble after 10 refinement iterations, contracted toward a feasible collision-free path.}
        \label{fig:ensemble_iter10}
    \end{subfigure}
    \caption{Evolution of the stochastic ensemble (15 candidates) during planning with an obstacle wall consisting of three stacked blocks between pickup and placement location. 
    Candidates are shown as green paths with via points as green spheres; they start with wide variability (\subref{fig:ensemble_init}) and contract to the collision-free region (\subref{fig:ensemble_iter10}).}
    \label{fig:ensemble_evolution}
\end{figure}


\section{Pose Estimation}
\label{sec:pose_estimation}
Our vision pipeline estimates the pose of blocks from RGB images $\mathcal{I}$ using fiducial markers. 
This choice provides a simple and robust fallback solution for the laboratory setup, ensuring reliable estimates under real-time constraints, 
even though the generality of marker-based approaches is limited.

Given a calibrated camera image $\mathcal{I}$ with intrinsics $\vec{K}$ and distortion parameters, 
we detect ArUco markers $\mathcal{M}$ \cite{Aruco} and estimate their pose $\vec{H}_\mathcal{C}^\mathcal{M}$ using the IPPE PnP algorithm \cite{IPPE}.
With the fixed hand–eye calibration $\vec{H}_\mathcal{T}^\mathcal{C}$ and the robot forward kinematics $\vec{H}_{0}^\mathcal{T}(\vec{q})$, 
the marker pose in the robot base frame is obtained as
\begin{equation}
\vec{H}_{0}^\mathcal{M} = \vec{H}_{0}^\mathcal{T}(\vec{q}) \vec{H}_\mathcal{T}^\mathcal{C} \vec{H}_\mathcal{C}^\mathcal{M} \Rightarrow\;
\big(
\vec{p}_{0}^{\mathcal{M}}, \vec{r}_{0}^{\mathcal{M}} \big) \Comma
\end{equation}
with position $\vec{p}_{0}^{\mathcal{M}} \in \mathbb{R}^3$ and orientation $\vec{r}_{0}^{\mathcal{M}} \in \mathbb{H}$ (unit quaternion).

Since the block motion is unknown, we adopt a constant-velocity motion prior as a generic assumption. 
The position $\vec{p}_{0}^{\mathcal{M}}$ is filtered with a discrete Kalman filter on the state 
$\hat{\vec{x}}_{p,k}=\transvec{\vec{p}_{0,k}^{\mathcal{M}},\,\vec{v}_{0,k}^{\mathcal{M}}}$, 
while the orientation $\vec{r}_{0}^{\mathcal{M}}$ is smoothed using a multiplicative EKF (MEKF) on $\mathrm{SO}(3)$ with quaternion error representation \cite{MEKF,SO3}. 
Both filters run at the camera rate using the measured frame interval $\Delta t_k$.

The filtered 6D poses are fed into the world model (see Fig.~\ref{fig:system_overview}) 
and serve as goal references for the path planner, which in turn updates the trajectory executed by the MPC.


\section{Laboratory Setup}
\label{sec:laboratory_setup}
The experimental platform comprises a KUKA LBR iiwa 14 R820 equipped with a Robotiq 2F-85 parallel-jaw gripper and two passive wrist DoFs. 
The unactuated coordinates $q_8$ and $q_9$ correspond to the relative roll and pitch between the robot end-effector and the gripper frame. 
These angles are inferred from a pair of IMUs (ADIS16460, Analog Devices) rigidly mounted on the end-effector and on the gripper, respectively. Raw angular velocities are first debiased; orientation estimates are then obtained using a Madgwick filter \cite{MaH11a}. Let $\vec{R}_{\mathcal{W}}^\text{I1}$ and $\vec{R}_{\mathcal{W}}^\text{I2}$ denote the orientation (rotation matrices) of the end-effector-mounted and gripper-mounted IMUs in the inertial frame. The relative rotation is computed as
\begin{equation}
\vec{R}_\text{I1}^\text{I2} = \transpose{ \left( \vec{R}_{\mathcal{W}}^\text{I1} \right) } \vec{R}_{\mathcal{W}}^\text{I2} \Comma
\end{equation}
from which the roll and pitch components are extracted to define $q_8$ and $q_9$. The IMU sampling rate is \SI{500}{\hertz}. A RealSense D405 depth camera is rigidly co-located with the gripper and operated at \SI{15}{\hertz} for close-range perception and ArUco-based pose estimation.

All device drivers for the IMUs and the camera run on a Raspberry~Pi~4 (Ubuntu, ROS~2). The Madgwick orientation filter, ArUco pose filtering, task sequencer, path planner, and the model predictive controller (MPC) execute on a workstation (Ubuntu~22.04, Intel Core i7-12700K, \SI{32}{\giga\byte} RAM) running ROS~2 with Eclipse Cyclone DDS as middleware. Hard real-time joint control is deployed on a Beckhoff TwinCAT PC at $T_\text{c}=\SI{125}{\micro\second}$ (\SI{8}{\kilo\hertz}); ROS~2 and TwinCAT communicate via UDP, and TwinCAT interfaces with the robot over EtherCAT.

% \begin{table}[h]
%     \centering
%     \caption{MPC weights used in experimental validation.}
%     \label{tab:weighting_matrices}
%     \begin{tabular}{cc}
%         \toprule
%         \textbf{Weight} & \textbf{Value} \\
%         \midrule
%         $\vec{Q}_{\text{pos}}$ & $200 \II_3$  \\
%         $Q_{\text{rot}}$ & $1000$ \\
%         $\vec{Q}_{\vec{q}}$ & $\text{diag}([0.01, 0.01, 0.5, 0.01, 0.5, 0.01, 0.01, 0.01, 0.01])$ \\ 
%         $\vec{Q}_{\dot{\vec{q}}}$ & $\text{diag}([0.1, 0.1, 1.0, 0.1, 1.0, 0.01, 0.01, 1.0, 1.0])$ \\
%         $Q_s$ & $0.3 \eta$ \\
%         $Q_{\dot{s}}$ & $5$ \\
%         $\vec{R}_{\vec{u}}$ & $0.1 \II_7$ \\
%         $R_v$ & $5$ \\
%         \bottomrule
%     \end{tabular}
% \end{table}
% Table \cref{tab:weighting_matrices} lists the weights in \cref{eq:lagrange_cost} used during the experiments.
The weights in \cref{eq:lagrange_cost} were tuned empirically, with high values on position and orientation tracking ($\vec{Q}{\text{pos}}, Q{\text{rot}}$) to ensure accuracy, and small posture and velocity regularization terms to stabilize redundancy, thereby balancing path-tracking precision, sway damping, and control effort in the experimental setup. 
The path parameter weight is scaled according to the path's length $\eta = \frac{1}{\max(\|\vec{p}_e - \vec{p}_s\|_2, 0.1)}$ with the path's start and end position $\vec{p}_s$ and $\vec{p}_e$, respectively. 
The horizon length in \cref{eq:ocp} is chosen as $N = 25$ steps, and the time discretization of the horizon is $T_\text{horizon} = \SI{0.03}{\second}$, which is fast enough for the passive joint dynamics and long enough horizon for smooth path-following.
The MPC runs with $T_\text{s}=\SI{20}{\milli\second}$ (\SI{50}{\hertz}) and publishes a sequence of joint-accelerations 
\begin{equation}
  \vec{u}_i \equiv \ddot{\vec{q}}_{\text{d}}(t_i), \quad t_i = t_0 + i\,T_\text{s}, \quad i=0,\ldots,N \FullStop
\end{equation}

Since the MPC and torque control loops operate at different cycle times 
($T_s=\SI{20}{\milli\second}$ vs.\ $T_c=\SI{125}{\micro\second}$), 
signal consistency requires explicit up- and down-sampling. Linear interpolation of accelerations ensures that the inner torque loop receives continuous, cycle-synchronous references, avoiding aliasing effects or discontinuities that would otherwise degrade performance.
%In the real-time environment, these trajectory points are upsampled from $T_\text{s}$ to $T_\text{c}$ by linear interpolation of the acceleration. 
For each control tick $k$ at $t_k = t_0 + k T_\text{c}$, let $i=\big\lfloor (t_k - t_0) / T_\text{s} \big\rfloor$ and
$ \lambda_k = \frac{t_k - t_i}{T_\text{s}} \in [0,1]$.
The commanded (reference) acceleration used by the torque loop is then
\begin{equation}
  \ddot{\vec{q}}_{\text{d}}[k] = (1-\lambda_k)\,\vec{u}_i + \lambda_k \vec{u}_{i+1} \FullStop
  \label{eq:acc_interp}
\end{equation}

The reference velocity and position at the control rate are obtained by semi-implicit (symplectic) Euler with step $T_\text{c}$
\begin{subequations}
\label{eq:ref_discrete_integration_tc}
\begin{align}
  \dot{\vec{q}}_{\text{d}}[k+1] &= \dot{\vec{q}}_{\text{d}}[k] + T_\text{c}\,\ddot{\vec{q}}_{\text{d}}[k] \Comma \\
  \vec{q}_{\text{d}}[k+1]       &= \vec{q}_{\text{d}}[k] + T_\text{c}\,\dot{\vec{q}}_{\text{d}}[k+1] \FullStop
\end{align}
\end{subequations}
These discrete-time references $\vec{q}_{\text{d}}[k]$, $\dot{\vec{q}}_{\text{d}}[k]$, $\ddot{\vec{q}}_{\text{d}}[k]$ are provided to the inner-loop inverse-dynamics (computed-torque) controller \cite{SiS09,spong2020robot}
\begin{equation}
  \vec{\tau}[k] = \bar{\vec{M}}_\text{a}(\vec{q}) \vec{v}[k] + \bar{\vec{C}}_\text{a}(\vec{q}, \dot{\vec{q}}) \dot{\vec{q}} + \bar{\vec{g}}_\text{a}(\vec{q}) \Comma
\end{equation}
with the virtual input
\begin{equation}
  \vec{v}[k] = \ddot{\vec{q}}_{\text{d}}[k] - \vec{K}_0 \left(\vec{q}-\vec{q}_{\text{d}}[k]\right) - \vec{K}_1 \left(\dot{\vec{q}}-\dot{\vec{q}}_{\text{d}}[k]\right) \Comma
  \label{eq:comp_torque}
\end{equation}
where $\vec{K}_0$ and $\vec{K}_1$ are positive definite diagonal gain matrices. 
The matrices $\bar{\vec{M}}_\text{a}(\vec{q})$, $\bar{\vec{C}}_\text{a}(\vec{q}, \dot{\vec{q}})$, and the vector $\bar{\vec{g}}_\text{a}(\vec{q})$ correspond to the actuated system in \cref{eq:split_system}, 
but with updated inertia parameters in the last link to account for the passive joint and gripper payload. 
Residual model errors due to motion are compensated by the low-level torque controller.

A lightweight world model (``digital twin'') maintains the state of movable workpieces, including their estimated 6D poses and assembly status. 
This world model parametrizes a MuJoCo simulation that is updated online and queried for collisions during path planning (see Fig.~\ref{fig:system_overview}). 
The simulation provides the collision environment used by the planner, ensuring that planning queries remain consistent with the real robot and workpieces. 
In this way, perception, planning, and control are tightly coupled through a unified representation of the scene.





\section{Experimental Validation}
\label{sec:results}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.35\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{graphics/block_pickup.png}
        \subcaption{Pickup.}
        \label{fig:exp_pickup}
    \end{subfigure}
    \hspace{0.05\columnwidth}
    \begin{subfigure}[b]{0.35\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{graphics/block_placement.png}
        \subcaption{Placement.}
        \label{fig:exp_placement}
    \end{subfigure}
    \caption{Block pickup and placement. 
    In (\subref{fig:exp_pickup}), a randomly placed block is grasped using vision-based pose estimation feedback. 
    In (\subref{fig:exp_placement}), the block is placed on top of an existing block at a predefined goal, consistent with nominal assembly targets.}
    \label{fig:experiment_pickup_placement}
\end{figure}

The framework was validated on block pickup and placement tasks with online vision updates. 
Figure~\ref{fig:experiment_pickup_placement} shows a representative sequence in which blocks are detected, grasped, and stacked. 
During execution, the vision system provides new pose updates at \SI{1}{\second} intervals, which are fused into the world model and passed as updated goal references to the planner. 
This relatively low update rate was chosen to make the effects of replanning and pose corrections clearly visible in the experiments. 
The underlying camera and filtering pipeline operate at \SI{15}{\hertz}, such that faster updates could be used in practice if required.


In all experiments, we use $K=3$ via points (start, goal, and one interior point). 
This minimal choice is sufficient for collision avoidance in the considered assembly scenarios while keeping the optimization lightweight. 
Determining the optimal number of via points for more complex tasks is an open question and left for future work.

Figure~\ref{fig:pose_plot} compares the reference trajectory (dashed) with the executed motion (solid), with replanning events marked by vertical dashed lines. 
The corresponding errors are shown in Fig.~\ref{fig:pose_error}, remaining below \SI{3}{\milli\metre} and \SI{3}{\degree} during slow approach phases, while transient deviations up to \SI{15}{\milli\metre} and \SI{5}{\degree} occur during faster motions (e.g.\ around $t=\SI{11}{\second}$). 
These values remain well within the tolerances required for block stacking in the laboratory setup.

The evolution of the path parameter $s$, its velocity $\dot{s}$, and acceleration $v$ (Fig.~\ref{fig:path_progress}) illustrates how the path-following MPC advances along the spline under real-time updates. 
Solver performance is summarized in Fig.~\ref{fig:acados_stats}: QP solve times remain below \SI{20}{\milli\second}, iteration counts stay moderate, and residuals confirm stable convergence of the RTI scheme. 
Together, these results demonstrate that the integrated framework achieves real-time feasibility on CPU hardware while maintaining sufficient accuracy for autonomous assembly.



\begin{figure}[t] % or [h], [b], depending on placement
    \centering
    \includegraphics[]{graphics/experiments/pose_plot.pdf}%
    \caption{Reference tracking during block pickup and placement (cf.\ \cref{fig:experiment_pickup_placement}). 
    Vertical dashed lines indicate replanning events (new path initialization), while dotted lines mark vision updates (goal corrections from pose estimation). 
    Top: Cartesian position components $x$ (red), $y$ (green), and $z$ (blue), with solid lines showing executed motion and dashed lines the reference path. 
    Bottom: yaw angle $\psi$, executed (solid) vs.\ reference (dashed).}
    \label{fig:pose_plot}
\end{figure}

\begin{figure}[t] % or [h], [b], depending on placement
    \centering
    \includegraphics[]{graphics/experiments/pose_error_plot.pdf}%
    \caption{Pose error during block pickup and placement. 
    Top: Cartesian position errors $\tilde{x}$ (red), $\tilde{y}$ (green), and $\tilde{z}$ (blue). 
    Bottom: yaw angle error $\tilde{\psi}$. 
    All errors are computed as the difference between executed and reference trajectories shown in \cref{fig:pose_plot}.}
    \label{fig:pose_error}
\end{figure}

\begin{figure}[t] % or [h], [b], depending on placement
    \centering
    \includegraphics[]{graphics/experiments/path_progress_plot.pdf}%
    \caption{Path progress during block pickup and placement. 
    Top: path parameter $s$ (solid: executed, dashed: reference; the reference ramps linearly from $0$ to $1$ for each new path to avoid discontinuities). 
    Middle: path velocity $\dot{s}$. 
    Bottom: path acceleration $v$, the additional control input of the augmented MPC formulation in \cref{sec:control}.}
    \label{fig:path_progress}
\end{figure}

\begin{figure}[t] % or [h], [b], depending on placement
    \centering
    \includegraphics[]{graphics/experiments/acados_stats_plot.pdf}%
    \caption{MPC performance metrics during block pickup and placement. 
    Top: computation times, with $t_\text{total}$ the overall MPC iteration time and $t_\text{QP}$ the QP solver time. 
    Middle: number of QP solver iterations per MPC step. 
    Bottom: convergence residuals, where $r_\text{stat}$ measures first-order optimality (gradient norm) and $r_\text{eq}$ the satisfaction of system dynamics constraints.}
    \label{fig:acados_stats}
\end{figure}



\Cref{fig:obstacle_avoidance} shows a sequence in which blocks are picked up on one side of an obstacle wall and stacked on the opposite side. The accompanying video provides a clearer view of this experiment, in particular, the gripper re-adjustments during pickup based on vision feedback.


\begin{figure}[htbp]
    \centering
    % Erste Reihe
    \begin{subfigure}[b]{0.3\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{graphics/wall_seq1.png}
        \caption{First pick up.}
        \label{fig:img1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{graphics/wall_seq2.png}
        \caption{Traverse.}
        \label{fig:img2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{graphics/wall_seq3.png}
        \caption{First placement.}
        \label{fig:img3}
    \end{subfigure}
    
    \vspace{0.5cm} % Abstand zwischen den Reihen
    
    % Zweite Reihe
    \begin{subfigure}[b]{0.3\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{graphics/wall_seq4.png}
        \caption{Second pick up.}
        \label{fig:img4}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{graphics/wall_seq5.png}
        \caption{Traverse.}
        \label{fig:img5}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{graphics/wall_seq6.png}
        \caption{Sec. placement.}
        \label{fig:img6}
    \end{subfigure}
    
    \caption{Assembly of blocks with an obstacle wall (cf.\ \cref{fig:ensemble_evolution}). 
    The wall consists of three stacked blocks separating pickup and placement locations. 
    Two blocks are transferred across the obstacle in sequence, each consisting of pickup, traverse, and placement.}
    \label{fig:obstacle_avoidance}
\end{figure}


\subsection{Sway Damping}
\Cref{fig:mpc_damping} illustrates the damping of passive joint oscillations achieved by the MPC controller. To evaluate performance, the gripper was manually perturbed to excite the sway angles $q_8$ and $q_9$. The controller was active from \SI{0}{\second} to \SI{15}{\second} and then deactivated, exposing the natural dynamics of the under-actuated joints. A damped-sine fit was applied to both cases, and the key parameters are summarized in \cref{tab:sway_damping}.

\begin{figure}[t] % or [h], [b], depending on placement
    \centering
    \includegraphics[]{graphics/damping/joint_plot_document.pdf}%
    \caption{Damping performance of the MPC controller. 
    The controller is active from $t=\SI{0}{\second}$ to $t=\SI{15}{\second}$, after which the natural lightly damped sway motion of the passive joints becomes visible. 
    Quantitative parameters of the fitted oscillations are reported in \cref{tab:sway_damping}.}
    \label{fig:mpc_damping}
\end{figure}


\begin{table}[htb]
    \centering
    \caption{Damping characteristics of DoF~9 with MPC active vs.\ inactive. 
    With MPC active, the decay rate and damping ratio increase by more than an order of magnitude, reducing the settling time from \SI{17.8}{\second} to below \SI{1}{\second}.}
    \label{tab:sway_damping}
    \begin{tabular}{lccc}
        \toprule
        & Decay rate $\sigma$ [1/s] & Damping ratio $\zeta$ & $T_{90\to10}$ [s] \\
        \midrule
        MPC on  & 2.50  & 0.23  & 0.88  \\
        MPC off & 0.12  & 0.013 & 17.8 \\
        \bottomrule
    \end{tabular}
\end{table}

The results highlight the exceptional damping achieved by the MPC controller: the effective damping ratio increases from $\zeta=0.013$ (barely damped) to $\zeta=0.23$, reducing the settling time by a factor of more than 20 (from \SI{17.8}{\second} to less than \SI{0.9}{\second}). Importantly, the oscillation frequency remains nearly unchanged (\SI{1.67}{\hertz} vs. \SI{1.54}{\hertz}), showing that the improvement is due to active damping rather than altered dynamics. This confirms that the MPC effectively suppresses passive joint sway, stabilizing the gripper motion in real time.


\section{Conclusion}
\label{sec:conclusion}
This paper presented a unified perception–planning–control framework for under-actuated manipulators with passive joints, realized on a laboratory-scale testbed designed to emulate articulated boom cranes. The integration of real-time vision feedback, collision-aware path generation, and nonlinear MPC enables closed-loop execution of assembly tasks under dynamic and cluttered conditions.  

Experiments on the testbed demonstrated autonomous block pickup, placement, and obstacle-avoidance assembly with online vision updates. The results confirmed both the real-time feasibility of the architecture and its ability to actively damp passive-joint sway, reducing settling times by more than an order of magnitude.  

By combining the framework with a laboratory-scale platform, we establish an efficient environment for developing autonomy concepts that can later be transferred to large-scale construction machinery. Future work will extend the vision system beyond fiducial markers, explore richer assembly tasks, and investigate integration with digital construction workflows.













==> graphics/system_block_diagram.tex <==

    \begin{tikzpicture}[
        node distance=2.5cm,
        block/.style={rectangle, draw, fill=blue!20, text width=2.2cm, text centered, rounded corners, minimum height=1.2cm},
        env/.style={rectangle, draw, fill=green!20, text width=2.2cm, text centered, rounded corners, minimum height=1.2cm},
        arrow/.style={->, >=stealth, thick},
        doublearrow/.style={<->, >=stealth, thick},
        vision/.style={->, >=stealth, thick, color=red},
        control/.style={<->, >=stealth, thick, color=blue},
        model/.style={->, >=stealth, thick, color=orange}
    ]
    
    % Nodes
    \node [block] (camera) {Camera};
    \node [block, right of=camera] (pose) {Pose Estimation};
    \node [env, below of=pose] (env) {Environment Model};
    \node [block, right of=pose] (planner) {Path Planner};
    \node [block, right of=planner] (mpc) {MPC};
    \node [block, right of=mpc] (robot) {Robot with Real-time Control};
    
    % Vision timing domain (30 Hz)
    \draw [vision] (camera) -- (pose) node[midway, above] {Images};
    \draw [vision] (pose) -- (planner) node[midway, above] {4D pose $\vec{\xi}$};
    \draw [vision] (robot.south) |- (pose.south) node[near end, right] {\small $H_{b,c}(\vec{q})$};
    
    % Model update timing
    \draw [model] (pose) -- (env) node[midway, right] {\small Pose updates};
    \draw [model] (robot.south) |- (env.south) node[near end, below] {\small Robot state};
    \draw [model] (env) -- (planner) node[midway, left] {\small Object poses};
    
    % Control timing domain (100+ Hz)
    \draw [control] (planner) -- (mpc) node[midway, above] {\small Path $\vec{c}_i$};
    \draw [control] (mpc) -- (robot) node[midway, above] {\small $\vec{q}$, $\dot{\vec{q}}$, $\ddot{\vec{q}}$};
    
    % Assembly input
    \draw [arrow] (planner.north) -- ++(0,0.8) node[above] {Assembly pose};
    
    % Legend
    \node [below=3cm of env] (legend) {
        \begin{tabular}{ll}
            \textcolor{red}{\rule{0.5cm}{0.1cm}} & Vision domain (30 Hz) \\
            \textcolor{orange}{\rule{0.5cm}{0.1cm}} & Model updates \\
            \textcolor{blue}{\rule{0.5cm}{0.1cm}} & Control domain (100+ Hz) \\
            \textcolor{black}{\rule{0.5cm}{0.1cm}} & External input
        \end{tabular}
    };
    
    \end{tikzpicture}

